ZO-Act: Efficient Zeroth-Order Fine-Tuning via One-Shot Activation-Informed Low-Rank Subspaces

Zeroth-order (ZO) optimization enables fine-tuning large language models when backpropagation is unavailable or memory-prohibitive, but existing methods often perturb full model weights or randomly constructed low-dimensional subspaces, yielding high-variance estimates and limited performance. We propose ZO-Act, an activation-informed ZO fine-tuning method that restricts perturbations to a fixed low-rank subspace derived from input activations. For each linear layer, ZO-Act computes a small activation basis once at initialization and optimizes only lightweight coefficient matrices using forward-only loss evaluations. This reduces the effective perturbation dimension, exposes explicit trainable variables compatible with momentum-based optimizers such as Adam, and naturally supports quantized LLM fine-tuning by keeping low-bit weights frozen. We analyze ZO-Act as zeroth-order optimization over a restricted coefficient space and show that perturbing the low-dimensional coefficients reduces both the variance-dependent convergence term and the finite-difference error of the ZO estimator, at the cost of a controlled subspace approximation bias that is mitigated by the low-rank structure of LLM activations and gradients. Experiments on Llama-3-8B, OPT-13B, and INT4 Llama-3-8B show consistent gains over strong ZO fine-tuning baselines across language understanding, question answering, and commonsense reasoning.

==> intro_back.tex <==
\section{Introduction}

Fine-tuning Large Language Models (LLMs) has become a standard paradigm for adapting them to downstream tasks. However, as LLMs scale to billions of parameters, the memory overhead of first-order (FO) optimizers like SGD and Adam, primarily due to the need for backpropagation and caching of activations, becomes prohibitive. Zeroth-order (ZO) optimization has emerged as a promising memory-efficient alternative, as it approximates gradients using only forward passes, thereby eliminating the need for backpropagation \citep{malladi2023fine}.

The foundational work introduced MeZO \citep{malladi2023fine}, a memory-efficient adaptation of the classical ZO-SGD algorithm. By employing the Simultaneous Perturbation Stochastic Approximation (SPSA) gradient estimator and an in-place implementation, MeZO demonstrated that ZO methods could fine-tune models with up to 66 billion parameters using the same memory footprint as inference, achieving performance comparable to FO fine-tuning on several tasks. However, subsequent research has identified key limitations of vanilla ZO-SGD, including slow convergence, high gradient estimation variance, and difficulty in handling the heterogeneous curvatures of the LLM loss landscape.

In response to these challenges, several enhanced ZO algorithms have been proposed. A comprehensive benchmarking study by Zhang et al. \citep{zhang2024revisiting} evaluated a wide spectrum of ZO methods—including ZO-SGD, ZO-Adam, ZO-SGD with Momentum (MMT), and ZO-SGD with Conservative updates—across various model families and tasks. Their work highlighted the critical role of task alignment and revealed a trade-off between algorithmic complexity, accuracy, and memory efficiency. They further proposed improvements such as block-wise descent and hybrid ZO-FO training.

To address the issue of heterogeneous curvatures, \citep{zhao2025second} proposed HiZOO, the first ZO optimizer to incorporate diagonal Hessian information. By estimating the curvature of the loss landscape with an additional forward pass, HiZOO acts as a preconditioner, adjusting the update magnitude for each parameter and significantly accelerating convergence and improving accuracy, particularly on large models like OPT-66B. Another line of research has focused on exploiting the intrinsic low-rank structure of gradients in LLM fine-tuning. Chen et al. \citep{chen2025enhancing} introduced LOZO, which employs a low-rank ZO gradient estimator. By using low-rank perturbation matrices, LOZO's gradient estimates better mirror the true FO gradients, leading to faster convergence and compatibility with memory-efficient momentum techniques. Similarly, Yu et al. \citep{yu2024subzero} proposed SubZero, which performs random subspace zeroth-order optimization via layerwise low-rank perturbations, significantly reducing gradient estimation variance. Park et al. \citep{park2025elucidating} further generalized this direction with Subspace-MeZO, establishing a unified theoretical framework for subspace perturbation in ZO optimization and proposing a block coordinate descent variant (MeZO-BCD) that achieves better trade-offs between convergence speed and memory usage.

Concurrently, sparsity has been identified as a powerful mechanism to improve ZO fine-tuning. Liu et al. \citep{liu2026sparse} introduced S-MeZO (Sparse MeZO), which selectively updates only a small fraction of ``sensitive parameters'' identified by criteria such as the empirical Fisher information matrix. This extreme sparsity reduces computational overhead and enhances performance by lowering the variance of gradient estimates. Moreover, the sparse mask can be pre-computed and transferred across tasks, enabling efficient on-device personalization when combined with quantization. Beyond sparsity, alternative optimization paradigms have also been explored. For instance, ZO-Muon \citep{lang2026powering} adapts the Muon optimizer—originally designed for first-order training—to the zeroth-order setting, achieving competitive convergence with negligible additional memory cost. Meanwhile, attempts to integrate ZO methods with adaptive learning rate strategies have led to variants like ZO-Adam \citep{zhang2024revisiting}, though their effectiveness remains task-dependent.

Despite these advances, existing ZO fine-tuning methods still face a fundamental trade-off between variance reduction, memory efficiency, and implementation simplicity. Full-weight ZO methods are simple and memory-efficient but suffer from high estimator variance because perturbations are sampled in the full parameter space. Curvature-aware and structured ZO methods can improve optimization, but often require additional forward evaluations, auxiliary statistics, or nontrivial implementation mechanisms. Existing low-rank and subspace-based methods reduce the perturbation dimension, yet their subspaces are typically random or not explicitly tied to the data-dependent geometry of the model. Sparse methods further reduce the number of updated parameters, but they often require costly or task-specific pre-computation of sensitive parameter masks. In addition, the interaction between ZO fine-tuning and quantized LLMs remains underexplored: directly perturbing low-bit weights is not natural, while maintaining full-precision shadow weights undermines the memory advantage of quantization.

To bridge this gap, we propose ZO-Act, a one-shot activation-informed zeroth-order fine-tuning framework. ZO-Act uses a calibration batch to compute a fixed low-rank subspace from the input activations of each linear layer and performs ZO optimization only over a small coefficient matrix in this subspace. By aligning the perturbation space with dominant activation directions, ZO-Act provides a data-informed alternative to random subspaces while keeping the method simple and forward-only. The resulting framework reduces the perturbation dimension from the full weight space to a compact coefficient space, enables direct use of Adam on explicit trainable variables, and avoids storing or materializing full-weight perturbations. Since the pretrained or quantized backbone remains frozen throughout training, ZO-Act is also naturally compatible with low-bit LLMs, making forward-only fine-tuning more practical in memory-constrained deployment settings.


Our main contributions are summarized as follows:
\begin{itemize}
    \item We propose ZO-Act, an activation-informed zeroth-order adaptation method that computes a fixed low-rank subspace from input activations once at initialization and optimizes only a lightweight coefficient matrix. The fixed-subspace parameterization reduces the number of optimized parameters and exposes explicit trainable variables, making it natural to apply momentum-based optimizers such as Adam. Since the pretrained weights remains frozen and only the small full-precision adapter is updated, the method is also well suited for quantized LLM fine-tuning.

    \item We provide a theoretical analysis showing that ZO-Act reduces the dimension-dependent variance in Gaussian ZO gradient estimation by replacing full-weight perturbations with perturbations in the much smaller coefficient space. The analysis further characterizes the trade-off introduced by subspace restriction: ZO-Act achieves lower-variance updates while relying on the activation-informed subspace to capture the dominant gradient directions.


    \item Extensive experiments on Llama-3-8B, OPT-13B, and INT4 Llama-3-8B demonstrate that ZO-Act consistently outperforms strong ZO fine-tuning baselines across language understanding, question answering, and commonsense reasoning tasks.
\end{itemize}



\section{Background and Related Work}


Zeroth-order optimization addresses the minimization or
maximization of an objective function $f$ : $\mathbb{R}^n \rightarrow \mathbb{R}$ without the use of derivatives:
$$\min_{\forall x \in \mathbb{R}^n} f(x)$$
The gradient $\nabla f(x)$ at a point $x$ can be approximated as:
$$\hat{\nabla} f( \mat{x}):= \frac{1}{q}\sum_{i=1}^q\frac{f(\mat{x}+\mu \mat{u}_i)-f(\mat{x}-\mu \mat{u}_i)}{2\mu} \cdot \mat{u}_i$$
where $ \mat{u}_i\sim \mathcal{N}(0,I)$, and $\mu$ is a small scalar.

MeZO \citep{malladi2023fine} applies ZO to LLM fine-tuning, achieving memory savings at the cost of slower convergence.

==> main_analysis.tex <==
\subsection{Formal Statement and Proof of Theorem \ref{thm:zoact-convergence-informal}}
\begin{theorem}[Convergence of ZO-Act]
	\label{thm:zoact-convergence-full2}
	Let \(\phi(\beta)=F(\theta_0+U\beta)\), where \(\beta\in\mathbb R^k\) collects all trainable coefficient matrices. 
	Assume that \(F\) is \(L_F\)-smooth, \(U^\top U=I\), and \(\phi\) is lower bounded by \(\phi_k^{\inf}\). 
	At iteration \(t\), ZO-Act samples \(q\) independent Gaussian directions \(z_t^{(j)}\sim\mathcal N(0,I_k)\) and uses the one-sided estimator
	\[
	\widehat g_t
	=
	\frac{1}{q}
	\sum_{j=1}^{q}
	\frac{\phi(\beta_t+\mu z_t^{(j)})-\phi(\beta_t)}{\mu}
	z_t^{(j)} .
	\]
	Suppose the update is \(\beta_{t+1}=\beta_t-\eta\widehat g_t\). 
	If
	\[
	0<\eta\le \frac{1}{L_F} \min \left\{\frac{q}{4(k+1)}, 1\right\}
	,
	\]
	then
	\[
	\begin{aligned}
		\frac{1}{T}\sum_{t=0}^{T-1}
		\mathbb E\|\nabla\phi(\beta_t)\|^2
		\le\;&
		\frac{4D}{\eta T} +
		L_F^2\mu^2 k(k+2)(k+4),
	\end{aligned}
	\]
	where \(D=\phi(\beta_0)-\phi_k^{\inf}\).
	In particular, choosing \(\eta=\frac{1}{L_F} \min \left\{\frac{q}{4(k+1)}, 1\right\}\) gives
	\[
	\begin{aligned}
		\frac{1}{T}\sum_{t=0}^{T-1}
		\mathbb E\|\nabla\phi(\beta_t)\|^2
		\le\;&
		\frac{4L_FD}{T}
		\max\left\{\frac{4(k+1)}{q},1\right\} \\
		&+
		L_F^2\mu^2 k(k+2)(k+4).
	\end{aligned}
	\]
	Moreover, \(\mu=\frac{\sqrt D}{(k+2)\sqrt{L_FT}} \max \left\{\frac{4}{\sqrt{q}}, \frac{2}{\sqrt{k+2}}\right\}\) gives
\[
	\frac{1}{T}\sum_{t=0}^{T-1}
	\mathbb E\|\nabla\phi(\beta_t)\|^2
	\le
	\frac{8L_FD}{T}
	\max\left\{\frac{4(k+2)}{q},1\right\}.
\]
\end{theorem}

\begin{proof}
	Since \(F\) is \(L_F\)-smooth and \(U^\top U=I\), the restricted objective \(\phi(\beta)=F(\theta_0+U\beta)\) is also \(L_F\)-smooth. 
	Indeed, \(\nabla\phi(\beta)=U^\top\nabla F(\theta_0+U\beta)\), and hence
	\[
	\|\nabla\phi(\beta)-\nabla\phi(\beta')\|
	\le
	L_F\|\beta-\beta'\|.
	\]
	Let \(g_t=\nabla\phi(\beta_t)\). 
	For each Gaussian direction \(z_t^{(j)}\), define
	\[
	\widehat g_t^{(j)}
	=
	\frac{\phi(\beta_t+\mu z_t^{(j)})-\phi(\beta_t)}{\mu}
	z_t^{(j)},
	\]
	\[
	\widehat g_t=\frac{1}{q}\sum_{j=1}^{q}\widehat g_t^{(j)} .
	\]
	By \(L_F\)-smoothness of \(\phi\), for any \(z\),
	\[
	\phi(\beta_t+\mu z)
	=
	\phi(\beta_t)
	+
	\mu\langle g_t,z\rangle
	+
	R_t(z),
	\]
	\[
	|R_t(z)|\le \frac{L_F\mu^2}{2}\|z\|^2 .
	\]
	We write $
	\widehat g_t^{(j)}
	=
	a_t^{(j)}+b_t^{(j)}$,
	where 
	$a_t^{(j)}=\langle g_t,z_t^{(j)}\rangle z_t^{(j)}$ is unbiased,
	and 
	$b_t^{(j)}=\frac{R_t(z_t^{(j)})}{\mu}z_t^{(j)}$ is the bias.
	
	The bias satisfies \(\|b_t^{(j)}\|\le (L_F\mu/2)\|z_t^{(j)}\|^3\). 
	Let \(\bar a_t=q^{-1}\sum_{j=1}^{q}a_t^{(j)}\) and \(\bar b_t=q^{-1}\sum_{j=1}^{q}b_t^{(j)}\), so that \(\widehat g_t=\bar a_t+\bar b_t =g_t+\bar a_t-g_t+\bar b_t\), which we will use to split the variance of $\bar a_t-g_t$ and the bias term $\bar b_t$.
	
	We first lower bound the variance of $\bar a_t-g_t$. 
	Since \(z_t^{(j)}\sim\mathcal N(0,I_k)\), we have \(\mathbb E[a_t^{(j)}]=g_t\), and hence \(\mathbb E[\bar a_t]=g_t\).  
	For each Gaussian term,
	\[
	\mathbb E\|a_t^{(j)}\|^2
	=
	\mathbb E[\langle g_t,z\rangle^2\|z\|^2]
	=
	(k+2)\|g_t\|^2 .
	\]
	Therefore, since the \(a_t^{(j)}\)'s are independent and each has mean \(g_t\),
	\[
	\begin{aligned}
		\mathbb E\|\bar a_t- g_t\|^2
		&=
		\frac{1}{q}\mathbb E\|a_t^{(j)}-g_t\|^2 \\
		&=
		\frac{1}{q}( \mathbb E\|a_t^{(j)}\|^2-\|g_t\|^2)  \\
		&=
		\frac{k+1}{q}\|g_t\|^2 .
	\end{aligned}
	\]
	For the bias term, by its definition,
	\[
	\mathbb E\|\bar b_t\|
	\le
	\frac{1}{q}\sum_{j=1}^{q}\mathbb E\|b_t^{(j)}\|
	\le
	\frac{L_F\mu}{2}\mathbb E\|z\|^3 .
	\]
	It holds \(\mathbb E\|z\|^3\le (\mathbb E\|z\|^6)^{1/2}\) and \(\mathbb E\|z\|^6=k(k+2)(k+4)\). We define \(M_k=k(k+2)(k+4)\),
	Then \(\mathbb E\|\bar b_t\|\le (L_F\mu/2)\sqrt{M_k}\). 	
	Moreover, Jensen's inequality gives
	\[
	\mathbb E\|\bar b_t\|^2
	\le
	\frac{1}{q}\sum_{j=1}^{q}\mathbb E\|b_t^{(j)}\|^2
	\le
	\frac{L_F^2\mu^2}{4}M_k .
	\]

	Now we analyze progress of each iteration. By smoothness of \(\phi\), the update \(\beta_{t+1}=\beta_t-\eta\widehat g_t\) satisfies the following chain:
\[
\begin{aligned}
	\phi(\beta_{t+1})
	\le&
	\phi(\beta_t)
	-
	\eta\langle g_t,\widehat g_t\rangle
	+
	\frac{L_F\eta^2}{2}\|\widehat g_t\|^2 \\
	=& \phi(\beta_t)
	-\eta\langle g_t,\bar a_t-g_t\rangle-\eta\langle g_t,\bar b_t\rangle-\eta\| g_t\|^2\\
	&+
	\frac{L_F\eta^2}{2}\| g_t\|^2+ L_F\eta^2 \langle g_t, \bar a_t-g_t+ \bar b_t\rangle\\
	&+\frac{L_F\eta^2}{2}\|\bar a_t-g_t +\bar b_t\|^2\\
	\le& \phi(\beta_t)
	-\eta(1-L_F\eta)\langle g_t,\bar a_t-g_t\rangle\\
	&-\eta(1-L_F\eta)\langle g_t,\bar b_t\rangle-\eta(1-L_F\eta/2)\| g_t\|^2\\
	&+ L_F\eta^2 (\|\bar a_t-g_t\|^2 +\|\bar b_t\|^2);
\end{aligned}
\]
we split $\widehat g_t$ in the second equality, and combine alike terms and apply \(\|u+v\|^2\le 2\| u\|^2+2\|v\|^2\) in the last inequality.

	Taking expectation conditioned on $\beta_t$ (and $g_t$), assuming $\eta\in[0,1/L_F]$, and applying Cauchy-Schwarz inequality to $|\langle g_t,\bar b_t\rangle|\le(\|g_t\|^2+\|\bar b_t\|^2)/2$, we have
	\[
	\begin{aligned}
		&\mathbb E_t[\phi(\beta_{t+1})]\\
		\le&
		\phi(\beta_t)
		-0+\frac{\eta}{2}(1-L_F\eta)\|g_t\|^2 \\
		&+\frac{\eta}{2}(1-L_F\eta)\mathbb E_t\|\bar b_t\|^2-\eta\Big(1-\frac{L_F\eta}{2}\Big)\| g_t\|^2\\
		&+ L_F\eta^2  \mathbb E_t\|\bar a_t-g_t\|^2 + L_F\eta^2\mathbb E_t\|\bar b_t\|^2  \\
		\le&
		\phi(\beta_t)
		-\frac{\eta}{2}\|g_t\|^2 +\frac{\eta}{2}(1+L_F\eta)\frac{L_F^2\mu^2}{4}M_k\\
		&+ L_F\eta^2 \frac{k+1}{q}\|g_t\|^2,
	\end{aligned}
	\]
	where we gathered alike terms and substituted the bounds established above. 
	Rearranging, 
	\[
	\begin{aligned}
		&\frac{\eta}{4}\Big(2-4L_F\eta\frac{k+1}{q}\Big)\|g_t\|^2	\\	
		&\le
		\phi(\beta_t)
		-\mathbb E_t[\phi(\beta_{t+1})] +\frac{\eta}{8}(1+L_F\eta)L_F^2\mu^2M_k.
	\end{aligned}
	\]
	Let \(0<\eta\le \frac{1}{L_F} \min \left\{\frac{q}{4(k+1)}, 1\right\}\), so that \(4L_F\eta\frac{k+1}{q}\le 1\) and \(L_F\eta\le 1\), we have
	\[
	\frac{\eta}{4}\|g_t\|^2
	\le
	\phi(\beta_t)
	-
	\mathbb E_t[\phi(\beta_{t+1})]
	+
	\frac{\eta L_F^2\mu^2}{4}M_k .
	\]
	Taking total expectation and summing from \(t=0\) to \(T-1\), we get
	\[
	\frac{\eta}{4}\sum_{t=0}^{T-1}
	\mathbb E\|g_t\|^2
	\le
	\phi(\beta_0)-\mathbb E[\phi(\beta_T)]
	+
	\frac{\eta L_F^2\mu^2}{4}M_k T .
	\]
	Since \(\phi(\beta_T)\ge \phi_k^{\inf}\), dividing by \(\eta T/4\) yields
	\[
	\frac{1}{T}\sum_{t=0}^{T-1}
	\mathbb E\|\nabla\phi(\beta_t)\|^2
	\le
	\frac{4(\phi(\beta_0)-\phi_k^{\inf})}{\eta T}
	+
	L_F^2\mu^2M_k.
	\]
	This proves the theorem.
\end{proof}
